Konstruktor: A Strong Baseline for Simple Knowledge Graph Question Answering

While being one of the most popular question types, simple questions such as "Who is the author of Cinderella?", are still not completely solved. Surprisingly, even the most powerful modern Large Language Models are prone to errors when dealing with such questions, especially when dealing with rare entities. At the same time, as an answer may be one hop away from the question entity, one can try to develop a method that uses structured knowledge graphs (KGs) to answer such questions. In this paper, we introduce Konstruktor - an efficient and robust approach that breaks down the problem into three steps: (i) entity extraction and entity linking, (ii) relation prediction, and (iii) querying the knowledge graph. Our approach integrates language models and knowledge graphs, exploiting the power of the former and the interpretability of the latter. We experiment with two named entity recognition and entity linking methods and several relation detection techniques. We show that for relation detection, the most challenging step of the workflow, a combination of relation classification/generation and ranking outperforms other methods. We report Konstruktor's strong results on four datasets.

==> Tables/ner_res.tex <==
\vspace{-10pt}

\begin{table}[h!]
\small
\centering
\renewcommand{\arraystretch}{1}
\caption{Named Entity Recognition results in terms of Accuracy@1 on the SQ-WD (validation), Mintaka (validation) and RuBQ-en (test). The best scores are highlighted. *Subset of 1-hop questions.}
\scalebox{0.96}{
\begin{tabular}{l|c|c|c}
\toprule
\bf Training data      & \bf  SQ-WD          & \bf RuBQ-en*           & \bf  Mintaka*        \\ \midrule
SQ-WD                  & \textbf{0.908} & 0.349          & 0.187          \\
RuBQ                   & 0.091          & 0.531          & 0.364          \\
Mintaka                & 0.021          & 0.419          & \textbf{0.881} \\
SQ-WD+RuBQ             & 0.876          & 0.515          & 0.234          \\
SQ-WD+Mintaka         & 0.896          & 0.445          & 0.539          \\
RuBQ+Mintaka         & 0.031          & 0.481          & 0.847          \\
All & 0.898          & \textbf{0.543} & 0.839          \\ \bottomrule
\end{tabular}
}
\vspace{-20pt}

\label{ner_res}
\end{table}

==> Tables/results_sensitivity.tex <==

\begin{table}[h!]
% \resizebox{0.5\textwidth}{!}{
\small
\centering
\renewcommand{\arraystretch}{1.1}
\caption{Results sensitivity for each of the combination of selected components. "Classifier" refers to the case of classifier(all data+DB loss) from Table~\ref{rel_clf} and "generation" to relation generation case Table~\ref{rel_clf}. The best scores are highlighted. *Subset of 1-hop questions.}
\scalebox{0.96}{
\begin{tabular}{lc|c|c|c}
\toprule
        & \begin{tabular}[c]{@{}c@{}} \bf mGENRE\\ \bf classifier\end{tabular} & \begin{tabular}[c]{@{}c@{}} \bf BELA\\  \bf classifier\end{tabular} & \begin{tabular}[c]{@{}c@{}} \bf mGENRE\\ \bf generator\end{tabular} & \begin{tabular}[c]{@{}c@{}} \bf BELA\\ \bf generator\end{tabular} \\ \midrule
SQ-WD   & \textbf{59.13}                                             & 50.10                                                    & 57.49                                                     & 47.73                                                   \\
RuBQ-en*    & 34.69                                                      & 30.20                                                    & 47.33                                                     & \textbf{52.45}                                           \\
% Mintaka* &      19.71	&  20.88	&  21.47  &                                                    \textbf{31.47}                                          \\ 
\bottomrule
\end{tabular}
}
\vspace{-10pt}

% }
\label{sensitivity}
\end{table}
